PAAM: A Framework for Coordinated and Priority-Driven Accelerator Management in ROS 2

This paper proposes a Priority-driven Accelerator Access Management (PAAM) framework for multi-process robotic applications built on top of the Robot Operating System (ROS) 2 middleware platform. The framework addresses the issue of predictable execution of time- and safety-critical callback chains that require hardware accelerators such as GPUs and TPUs. PAAM provides a standalone ROS executor that acts as an accelerator resource server, arbitrating accelerator access requests from all other callbacks at the application layer. This approach enables coordinated and priority-driven accelerator access management in multi-process robotic systems. The framework design is directly applicable to all types of accelerators and enables granular control over how specific chains access accelerators, making it possible to achieve predictable real-time support for accelerators used by safety-critical callback chains without making changes to underlying accelerator device drivers. The paper shows that PAAM also offers a theoretical analysis that can upper bound the worst-case response time of safety-critical callback chains that necessitate accelerator access. This paper also demonstrates that complex robotic systems with extensive accelerator usage that are integrated with PAAM may achieve up to a 91\% reduction in end-to-end response time of their critical callback chains.

==> draft/5-Analysis.tex <==
\subsection{Admission Control}\label{sec:analysis}
For any new client, the PAAM server performs admission control to determine its acceptance. One approach would be to simply assess the utilization of clients' accelerator requests.
%, i.e., decline if the utilization exceeds 100\%. This can be used when lower-priority chains are allowed to miss deadlines for higher-priority chains. 
However, to guarantee end-to-end performance,
%to check rigorously whether the acceptance of the new client can satisfy its timing requirements and does not hamper the timeliness of existing clients, 
we derive the {\em worst-case response time of a chain} that includes callbacks accessing accelerators through PAAM. As mentioned in Sec.~\ref{sec:background}, we adopt the priority-driven chain execution mechanism of PiCAS~\cite{choi2021picas}. Hence, our approach extends the analysis from \cite{choi2021picas}, incorporating the delays induced by accelerator access. While PAAM supports various client executors, for analysis purposes, we follow the same assumptions as in \cite{choi2021picas}: clients use single-threaded executors, each statically assigned to a CPU core with a distinct real-time process priority. Our analysis focuses on chains with constrained deadlines. \uline{Proofs and detailed explanations are in our supplementary document.}

Let us consider a chain $\Gamma_c$ executing in one executor. This chain could be a sub-chain of a larger chain $\Gamma^*$ that spans across multiple executors on different CPU cores. We will first upper-bound the response time of $\Gamma_c$ and then show how the end-to-end response time of $\Gamma^*$ can be obtained. 

In PAAM, the key behavior rules that affect the request handling time for accelerator access are summarized as follows.
\begin{itemize}[leftmargin=*]
	\item R1: For each accelerator device, one server is created and runs on a dedicated CPU. Hence, different PAAM servers do not interfere with each other on both CPU and accelerator.
	\item R2: When an PAAM server receives a request, it is sent to one of $n$ buckets through priority downsampling and handled by the corresponding worker thread of the server. 
	\item R3: The worker thread executes requests in its bucket non-preemptively in the order of requests' chain priority.
	\item R4: If the server has multiple buckets, requests in a higher-priority (HP) bucket can preempt those in a lower-priority (LP) one.
\end{itemize}
R1 allows us to analyze the request handling time for one accelerator independent of other accelerators in the system. R2-R4 are resulted from our two-level hierarchical request management. By R2 and R3, a chain $\Gamma_c$'s request can be delayed by up to one request from an LP chain that the accelerator is already executing. R4 adds interference from HP chains during the handling time of $\Gamma_c$'s request.
In addition, there are two types of overhead to consider: (i) $\epsilon$, which is the overhead imposed on every request (accelerator segment) by the PAAM server ($\delta_c$ segments for $\Gamma_c$), and (ii) $\kappa$, which is the device-level preemption cost that can occur before and after each segment (at most $2\kappa$ per segment). We define $A_{i,j}^*=A_{i,j}+2\kappa$ to incorporate the preemption delay into the execution time of the $j$-th accelerator segment of a callback $\tau_i$. Based on this, the maximum time to complete all accelerator requests of the chain $\Gamma_c$ with overhead is given by:
\begin{equation}
    \label{eq:beta}
    H_{c}^* = H_c + 
     \delta_c\cdot \epsilon 
\end{equation}
where $H_c$ is the cumulative request handling time for all accelerator segments of $\Gamma_c$ under PAAM (incl. delay R2-R4).
%, and $\delta_c$ is the number of accelerator segments of $\Gamma_c$.

Before bounding the handling time $H_c$, let us analyze how many accelerator requests an PAAM server can receive from an interfering segment $\tau_{k,q}$ during an arbitrary time interval $t$. 

\begin{lemma}[arrival bound]\label{lm:req_arrival} 
	The maximum number of requests that an accelerator segment $\tau_{k,q}$ from a schedulable chain $\Gamma_{c'}$ can generate in an arbitrary interval $t$ is bounded by
	\begin{equation}\label{eq:req_arrival}
		\begin{split}
			\mu_{k,q}(t) & \gets
			\Big\lceil \frac{t}{T_{c'}} \Big\rceil +1 
		\end{split}
	\end{equation}
\end{lemma}
% \begin{proof}
% The requests of a segment $\tau_{k,q}$ are made in a periodic manner based on its chain period, with a possible jitter $j_1<T_{c'}$ due to that $\tau_{k,q}$ can start as soon as its preceding segment or callback completes. If the interval $t$ is aligned with the release time of the chain $\Gamma_{c'}$, this gives $ \lceil \frac{t+j_1}{T_{c'}}\rceil$ (recall $\mu()$ is not a response time test; it is to bound the number of arrivals of requests during $t$). However, as $t$ is an arbitrary interval, there can be {\em carry-in} execution of $\tau_{k,q}$ in the interval $t$ due to delayed execution. For instance, the start of the execution of $\tau_{k,q}$'s job can be delayed by other callbacks on the same executor (e.g., blocking or self-pushing effect of non-preemptive scheduling) or by OS-level preemption from HP executor processes on the same CPU core. While this may introduce a more number of jobs of $\tau_{k,q}$ in the interval $t$ than $\lceil \frac{t}{T_{c'}}\rceil$, it is known to be limited to most once in a schedulable system with the constrained deadline model~\cite{bertogna2008schedulability} and its effect can be taken into account as a jitter, i.e., $j_2<T_{c'}$. The sum of these jitters $j_1$ and $j_2$ cannot exceed $T_{c'}$ since $\Gamma_{c'}$ is schedulable, and therefore $ \lceil \frac{t+j_1+j_2}{T_{c'}}\rceil\le \lceil \frac{t}{T_{c'}}\rceil+1$. It is worth noting that the well-known self-pushing effect of non-preemptive scheduling can be upper bounded by at most one carry-in job in the interval $t$ because $\Gamma_c'$ is schedulable. 
% \end{proof}

To bound $H_c$, we follow the double-bounding approach~\cite{Kim_JSA18,kim2021addressing} that derives two separate but safe bounds and takes the minimum between them. 
We will present each approach in a respective subsection and then derive the response time analysis of a chain. We will use the following notation:
\begin{itemize}
	\item $hps(\tau_{i,j})$ (and $lps(\tau_{i,j})$): the set of accelerator segments that are from HP (and LP) chains than the chain of $\tau_{i,j}$ and use the same accelerator as $\tau_{i,j}$.
 %i.e., $\{\tau_{k,q} \in \Gamma_l| \pi(\Gamma_l) > \pi(\Gamma_c) \wedge r_{k,q} = r_{i,j}\}$ where $\pi(\Gamma_c)$ is the chain priority of $\Gamma_c$ and $r_{i,j}$ is the accelerator used by the segment $\tau_{i,j}$.
%	\item $lps(\tau_{i,j})$: the set of accelerator segments that are from LP chains than the chain of $\tau_{i,j}$ and use the same accelerator as $\tau_{i,j}$, i.e., $\{\tau_{k,q} \in \Gamma_l| \pi(\Gamma_l) < \pi(\Gamma_c) \wedge r_{k,q} = r_{i,j}\}$.
	\item $b(\tau_{i,j})$: the bucket of the PAAM server assigned to $\tau_{i,j}$. 
\end{itemize}

\subsubsection{{Bound by Per-segment Handling Time}}
First, the handling time $H_c$ of a chain can be obtained by calculating the handling time of each accelerator segment $\tau_{i,j}$, $H_{c,i,j}$, and then adding them up, i.e., $H_c=\sum_{\tau_i\in\Gamma_c}\sum_{1\le j \le \eta_i}H_{c,i,j}$. 
%Lemma~\ref{lm:max_waiting} formulates $H_{c,i,j}^w$.
\begin{lemma}[handling time per segment]  
The maximum handling time of the $j$-th accelerator segment of a callback $\tau_i \in \Gamma_c$ under PAAM is upper-bounded by the recurrence:
\begin{equation}\label{eq:1}
\resizebox{.94\linewidth}{!}{$
\begin{split}
    H_{c, i, j} & \gets A_{i,j}^* + \!\!\!\!\!\!\!    
    \max_{\substack{\tau_{k,q} \in lps(\tau_{i,j}) \\\wedge b(\tau_{k,q}) = b(\tau_{i,j})}}{\!\!\!\!\!\!A_{k,q}^*}     
    +\!\!\!\!\!\sum_{\substack{\tau_{k,q} \in hps(\tau_{i,j})}}{\!\!\!\!\!\!\!\!\!\! \mu_{k,q}(H_{c,i,j}) \! \cdot \! A_{k,q}^*}
\end{split}$}\hspace{-10pt}
\end{equation}
The recurrence starts with the first two terms. %($H_{c,i,j} = \max{A_{k,q}^*}+A_{i,j}^*$).
\label{lm:max_waiting}
\end{lemma}
% \begin{proof}
% As explained earlier, the handling time $H_{c,i,j}$ of the accelerator segment of $\tau_{i,j}$ is determined by three factors. First, $\tau_{i,j}$'s own execution time inflated with the preemption cost, $A_{i,j}^*$. Secondly, blocking time occurs when the accelerator is already handling a request from an LP chain in the same bucket, which is the first term of the equation. Note that those in other buckets do not cause blocking because they can be preempted (recall PAAM creates more than one bucket only when the accelerator supports device-level preemption). Thirdly, an additional delay is imposed by HP requests during the handling time of $H_{c,i,j}$, the number of which is bounded by $\mu_{k,q}(H_{c,i,j})$. Therefore, the delay caused by requests from $\Gamma_h$ is bounded by { $\sum\mu_{k,q}(H_{c,i,j})\cdot A_{k,q}^*$}, and the maximum handling time can be obtained by adding these three factors.
% \end{proof}

\subsubsection{{ Bound by Per-chain Handling Time}}
Unlike the first approach, the second approach takes into account the total amount of interfering requests during the chain $\Gamma_c$'s execution. 

\begin{lemma}[handling time per chain job]
The maximum handling time of all accelerator segments from all callbacks of a chain $\Gamma_c$ under PAAM is upper-bounded by:
\begin{equation}\label{eq:2}
\resizebox{.94\linewidth}{!}{$
\begin{split}
    H_{c} & \!\gets\!\!\!
    \sum_{\tau_{i,j}\in\Gamma_c}\!\!\!
    \Big(\! A_{i,j}^*+\!\!\!\!\!\! \max_{\substack{\tau_{k,q} \in lps(\tau_{i,j}) \\\wedge b(\tau_{k,q}) = b(\tau_{i,j}) }}{\!\!\!\!\!\!A_{k,q}^*} 
    \Big) 
    \! + \!\!\!\!\!\!\sum_{\substack{\tau_{k,q} \in hps(\tau_{i,j})}}{\!\!\!\!\!\!\!\!\!\mu_{k,q}(R_c)\! \cdot \! A_{k,q}^*}
\end{split}$}\hspace{-10pt}
\end{equation}
where $R_c$ is the response time of $\Gamma_c$. This can be solved during the iterative calculation of $\Gamma_c$'s response time $R_c$ given next. 
\label{lm:max_waiting2}
\end{lemma}
% \begin{proof}
% Each accelerator request made by a segment $\tau_{i,j}$ of $\Gamma_c$ may experience blocking time from an LP request in the same bucket, and the total blocking time for $\Gamma_c$ can be bounded by the summation of each blocking time for all segments of $\Gamma_c$, as shown in the first term that also includes the execution time of $\Gamma_c$'s own requests. During $\Gamma_c$'s response time, the number of requests from an HP chain $\Gamma_h$ is bounded by $\mu_{k,q}(R_c)$, and the second term of the equation bounds the delay from HP chains.
% \end{proof}

It is worth noting that the two approaches given in Lemmas~\ref{lm:max_waiting} and \ref{lm:max_waiting2} do not dominate each other. While the blocking time from LP chains is the same, the amount of interference from HP chains is different. %For instance, if the number of accelerator segments of a chain $\Gamma_c$ under analysis is relatively small, Lemma~\ref{lm:max_waiting} can give a tighter bound since it only considers HP interference during the segments' handling time; in the opposite case, Lemma~\ref{lm:max_waiting2} can give a better result since its second term is not subject to the number of segments $\Gamma_c$ has. Since both approaches upper bounds the handling time, we can take the minimum between them to obtain the handling time $H_c$, and use this in Eq.~\eqref{eq:1} to compute $H_c^*$, the time to complete all accelerator requests of $\Gamma_c$ with overhead.

As mentioned before, we analyze a chain or sub-chain $\Gamma_c$ that has all of its callbacks running on a single executor, and then extend it to multiple executors. %discuss how chains spanning across multiple executors can be analyzed.
We use the following notation to specify other interfering chains:
\begin{itemize}
	\item $hp(\Gamma_c)$ (and $lp(\Gamma_c)$): the set of HP (and LP) chains than $\Gamma_c$ running in the same executor as $\Gamma_c$. %, i.e., $\{\Gamma_l| \Gamma_l \in e(\Gamma_c) \land \pi(\Gamma_l) > \pi(\Gamma_c) \}$ where $e(\Gamma_c)$ is the executor process of $\Gamma_c$.
	%\item $lp(\Gamma_c)$: the set of LP chains than $\Gamma_c$ running in the same executor as $\Gamma_c$, i.e., $\{\Gamma_h| \Gamma_h \in e(\Gamma_c) \land \pi(\Gamma_h) < \pi(\Gamma_c)\}$.
	\item $hpp(\Gamma_c)$: the set of chains running in executors on the same CPU as $e(\Gamma_c$) and with higher process priority than $e(\Gamma_c)$.%, i.e., $\{\Gamma_h| core(e(\Gamma_h))=core(e(\Gamma_c)) \land \pi(e(\Gamma_h)) > \pi(e(\Gamma_c))\}$ where $core(e(\Gamma_h))$ is the CPU core of the executor $e(\Gamma_h)$.
\end{itemize}

% Let us first review the response time test of PiCAS~\cite{choi2021picas}, the priority-driven execution mechanism adopted in PAAM. 
% \begin{lemma}[chain with no accelerator segment~\cite{choi2021picas}]\label{lm:wcrt_picas}
% The worst-case response time (WCRT) of a chain $\Gamma_c$ without any accelerator segment under the priority-driven chain execution mechanism is bounded by the following recurrence: 
% \begin{equation}\label{eq:wcrt_picas}
% \resizebox{.94\linewidth}{!}{$
% \begin{split}
%     R_{c} \gets & \mathcal{B}_c  +\mathcal{E}_c
%     + \!\!\!\! \sum_{\substack{\Gamma_h \in hp(\Gamma_c)}} \!\!\!\!\!\! \mu_h(R_c) \cdot \mathcal{E}_h 
%     + \!\!\!\! \sum_{\Gamma_h \in hpp(\Gamma_c)}\!\!\!\!\!\! \mu_h(R_c)\cdot  \mathcal{E}_h 
% \end{split}$}\hspace{-10pt}
% \end{equation}
% where $\mathcal{B}_c=\max_{\Gamma_l\in lp(\Gamma_c)}\max_{\substack{\tau_j \in \Gamma_l}} E_j$ is the blocking time from an LP chain, 
% $\mathcal{E}_c =\sum_{\substack{\tau_i\in \Gamma_c }}{E_i}$ is the sum of WCET of all callbacks of $\Gamma_c$, and $\mu_h(R_c)=\lceil \frac{R_c}{T_h} \rceil +1 $ is analogous to Lemma~\ref{lm:req_arrival}. The recurrence starts with the first two terms.%, i.e., $R_{c} = \mathcal{B}_c + \mathcal{E}_c$.
% \end{lemma}
%In the above analysis, the first term captures blocking time due to the non-preemptive callback scheduling of ROS 2. As the priority-driven execution mechanism prevents further execution of callbacks from LP chains until $\Gamma_c$ completes, there can be at most one blocking from a callback of an LP chain on the same executor. The second term $\mathcal{E}_c$ is the execution time of $\Gamma_c$ itself. The third term is the interference from HP chains on the same executor. An interesting part is the fourth term. This captures the fact that the executor process of $\Gamma_c$ can be preempted by other HP executor processes running on the same CPU core (i.e., OS-level preemption), each of which is activated by the arrival of any chain it has. 

We now derive the response time of a chain $\Gamma_c$ with accelerator segments under the PAAM framework by extending the one given by PiCAS~\cite{choi2021picas}. The PiCAS analysis takes into account: (i) blocking time from an LP chain due to the non-preemptive callback scheduling of ROS 2, given by $\mathcal{B}_c=\max_{\Gamma_l\in lp(\Gamma_c)}\max_{\substack{\tau_j \in \Gamma_l}} E_j$, (ii) $\Gamma_c$'s own execution time, i.e., the sum of WCET of all callbacks of $\Gamma_c$ given by $\mathcal{E}_c =\sum_{\substack{\tau_i\in \Gamma_c }}{E_i}$, (iii) interference from HP chains on the same executor, and (iv) preemption by HP executors on the same CPU.
On top of these, the additional factors we need to consider are: (v) accelerator segment execution time $H_c$ of the chain $\Gamma_c$ under analysis, (vi) interference due to accelerator usage of HP chains on the same executor, and (vii) accelerator usage of HP executors on the same CPU core.

\begin{theorem}
The worst-case response time (WCRT) of a chain $\Gamma_c$ with accelerator segments under the PAAM framework is bounded by the following recurrence: 
\begin{equation}
\begin{split}
R_{c} &\gets  \mathcal{B}_c+\mathcal{E}_c+H_c^*
    + \sum_{\substack{\Gamma_h \in hp(\Gamma_c)}}\mu_h(R_c)\cdot (\mathcal{E}_h+H_h^*) \\ 
    &+\sum_{\Gamma_h \in hpp(\Gamma_c)}\mu_h(R_c)\cdot ( \mathcal{E}_h +spin(\Gamma_h))
\label{eq:wcrt_chain}
\end{split}
\end{equation}
where 
%$\mathcal{B}_c=\max_{\Gamma_l\in lp(\Gamma_c)}\max_{\substack{\tau_j \in \Gamma_l}} E_j$ is the blocking time from an LP chain, 
%$\mathcal{E}_c =\sum_{\substack{\tau_i\in \Gamma_c }}{E_i}$ is the sum of WCET of all callbacks of $\Gamma_c$, 
$\mu_h(R_c)=\lceil \frac{R_c}{T_h} \rceil +1 $ which is analogous to Lemma~\ref{lm:req_arrival}, 
$spin(\Gamma_h)= H_h^*$ if $\Gamma_h$ spins (busy waits) on the CPU while waiting for the completion of accelerator requests, and $spin(\Gamma_h)=
\delta_h\cdot \epsilon$ otherwise ($\Gamma_h$ suspends). The recurrence starts with the first three terms, i.e., $R_{c} = \mathcal{B}_c + \mathcal{E}_c + H_c^*$.
\label{lm:wcrt_task}
\end{theorem}
% \begin{proof}
% The equation is an extension of Eq.~\eqref{eq:wcrt_picas}. The term $H_c^*$ is the handling times for accelerator segments of $\Gamma_c$ itself. For HP chains running in the same executor as $\Gamma_c$ (the first summing term), additional interference caused by each instance of an HP chain $\Gamma_h$ due to its accelerator execution time $H_h^*$ needs to be considered. This is because, while any accelerator request of a callback of $\Gamma_h$ is being handled by PAAM, this callback remains uncompleted and the executor cannot execute any other callback. On the other hand, for chains running on other executors with higher process priority on the same CPU core, the amount of additional interference per chain instance depends on whether that chain spins or suspends during accelerator requests.
% In case of spinning, the executor actively consumes CPU cycles, so all components of $H_h^*$ given by Eq.~\eqref{eq:beta} need to be taken into account. In case of suspension, the corresponding executor suspends and the interference is limited to  $\delta_h \cdot \epsilon$, which is the total overhead caused by PAAM. In the literature, self-suspending behavior of an HP task is known to introduce additional penalty to its LP tasks and such penalty can be bounded by a jitter term~\cite{bletsas2015errata,chen2019many}. As $\mu_h(R_c)$ already takes into account the maximum possible jitter for the constrained deadline model, no additional penalty needs to be considered.
% As there is no other source of interference or blocking delay possible for $\Gamma_c$, the summation of these terms can upper bound the response time.
% \end{proof}
As known in the literature~\cite{von2021realistic,davis2010quantifying}, a sufficient schedulability test for non-preemptive scheduling can be obtained by adding the blocking term to the response time test for preemptive scheduling, and our analysis follows this approach. This is safe but pessimistic. We believe a tighter analysis could be derived by considering the level-$i$ active period that can precisely capture the self-pushing phenomenon of non-preemptive scheduling.

\medskip\noindent\textbf{Processing Chain over Multiple Executors.}
Using Theorem~\ref{lm:wcrt_task}, we can obtain the end-to-end latency of a chain $\Gamma^*$ that consists of multiple sub-chains $\Gamma_c\in \Gamma^*$, { each of which is executed by different executors.} This can be directly computed by adding all the response times of sub-chains with {  communication cost $\epsilon'$ ($ \epsilon'< \epsilon$; see Sec.~\ref{sec:eval} for the breakdown of the PAAM overhead $\epsilon$)}, i.e., $R^*=\sum_{\Gamma_c\in \Gamma^*}R_c+\epsilon$. This works because, although subsequent sub-chains may experience release jitters when the preceding sub-chains finish earlier than their WCRT, the negative impact of such jitters on LP chains has been already considered as a carry-in ({ ``+1'' in Lemma~\ref{lm:req_arrival}}). This approach has been used by other prior work for ROS 2~\cite{choi2021picas, casini2019response}.

%\medskip\noindent\textbf{Device-level Preemption Overhead.} One may wonder how the WCET of an accelerator segment estimated in isolation, $A_{i,j}$, can be used with our analysis if the accelerator supports device-level preemption, e.g., GPUs. Suppose an upper-bound on this overhead is $\kappa$. This overhead can occur before and after the execution of each accelerator segment (to preempt and resume a lower-priority segment), so there can be at most $2\kappa$ per segment and this can be easily captured in the analysis by inflating each accelerator segment's execution time by $2\kappa$, i.e., $A_{i,j}+2\kappa$. In case of the Nvidia GPU, $\kappa$ is mainly due to the pixel-level and thread-level preemption delay and GPU-context switching overhead and this already happens on the default Nvidia driver due to its time-sliced scheduling of GPU contexts~\cite{capodieci2018deadline}. To account for this delay, one can estimate $\kappa$ by calculating the context size or taking measurements, as discussed in \cite{capodieci2018deadline}. Note that $\kappa$ exists only if device-level preemption is supported on hardware and two or more buckets exist; if not, e.g., TPUs, $\kappa=0$.

==> draft/6-Evaluation-Long.tex <==
\section{Evaluation}\label{sec:eval}
In this section, we assess the effectiveness of our proposed framework over the state-of-the-art and explore the performance characteristics and associated overhead. The evaluation was done on the Nvidia Jetson AGX Xavier platform that has 1 integrated GPU and 1 Google Coral Edge TPU. We configured all CPU and accelerator cores to run at the maximum frequency and disabled dynamic clock frequency scaling to minimize measurement fluctuations. Each experiment was run, uninterrupted, for 10 minutes at a time.\footnote{\blue The source code of our implementation is available at https://github.com/rtenlab/reference-system-paam.git}
%\uline{The source code of our implementation will be released after the review process.} 

%In this section, we assess the effectiveness of our proposed framework, specifically implemented for systems equipped with Nvidia GPUs and Coral Edge TPUs\footnote{The source code is available at XXX (redacted for double-blind review).} We compare the end-to-end latencies of critical processing chains, which are accelerated by GPU and TPU, utilizing our framework against those operating on the PiCAS-enabled framework~\cite{choi2021picas} and the default ROS 2 scheduler. %We further scrutinize the efficacy of our framework through realistic scenarios, modeling complex robotic systems comprising multiple interconnected callbacks. Overall, our evaluation provides a compelling testament to the advantages of our proposed framework and its potential for improving the predictability and reliability of GPU-accelerated robotic applications.

%The evaluation was done on the Nvidia Jetson AGX Xavier platform which has 8 CPU cores and 1 integrated GPU. {\blue To demonstrate support for multiple types of accelerators, we also interfaced the AGX with the Coral Edge TPU Accelerator. During experiments, we configured all CPU and accelerator cores to run at the maximum frequency and disabled dynamic clock frequency scaling. The PAAM server executor was pinned to core 0 with real-time priority in Linux. The worker threads for the GPU were also assigned to CPU core 0, and the worker threads for the TPU were assigned to core 1, each maintaining real-time priority in Linux. }Each case study was run, uninterrupted, for 10 minutes at a time, with tens of thousands of requests logged. 

\begin{figure}[t]
	\centering
	\subfloat{
		\includegraphics[width=\linewidth]{figures/case_study.pdf}
        }
	%	\vspace*{-1mm}
	%\caption{Execution Flow}
        \caption{Chain configuration of GPU-enabled robotic system}
	\label{fig:case_study}
\end{figure}

% \begin{table}[]
% %\resizebox{.95\textwidth}{!}{%
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|c|c|c|r|r|r|r|r|r|r|} 
% \hline
% \multirow{3}{*}{\textbf{Chain}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Chain}\\\textbf{Priority}\end{tabular}} & \multirow{3}{*}{\textbf{\# Callbacks}} & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Total }\\\textbf{CPU time}\\\textbf{ (ms)}\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Total }\\\textbf{GPU time }\\\textbf{ (ms)}\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Period}\\\textbf{ (ms)}\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\textbf{Response~Time~(ms)}}}                                                                                                          \\ 
% \cline{7-10}
%                                 &                                                                                            &                                        & \multicolumn{1}{c|}{}                                                                                                            & \multicolumn{1}{c|}{}                                                                                                             & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{2}{c|}{\textbf{Single bucket}}                                     & \multicolumn{2}{c|}{\textbf{Multi bucket}}                                       \\ 
% \cline{7-10}
%                                 &                                                                                            &                                        & \multicolumn{1}{c|}{}                                                                                                            & \multicolumn{1}{c|}{}                                                                                                             & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{1}{c|}{\textbf{Analysis}} & \multicolumn{1}{c|}{\textbf{Observed}} & \multicolumn{1}{c|}{\textbf{Analysis}} & \multicolumn{1}{c|}{\textbf{Observed}}  \\ 
% \hline
% \textbf{Chain 1}                & 6                                                                                          & 2                                      & 8                                                                                                                                & 20                                                                                                                                & 120                                                                                                           & 48                                     &                 43                       & 48                                     & 43                                     \\ 
% \hline
% \textbf{Chain 2}                & 5                                                                                          & 3                                      & 19                                                                                                                               & 30                                                                                                                                & 120                                                                                                           & 119                                    &                  99                      & 89                                     & 82                                      \\ 
% \hline
% \textbf{Chain 3}                & 4                                                                                          & 4                                      & 26                                                                                                                               & 40                                                                                                                                & 220                                                                                                           & 206                                    &                 125                       & 166                                    & 113                                     \\ 
% \hline
% \textbf{Chain 4}                & 3                                                                                          & 3                                      & 14                                                                                                                               & 30                                                                                                                                & 260                                                                                                           & 254                                    &                   104                     & 224                                    & 113                                     \\ 
% \hline
% \textbf{Chain 5}                & 2                                                                                          & 3                                      & 10                                                                                                                               & 30                                                                                                                                & 320                                                                                                           & 310                                    &                  138                      & 280                                    & 136                                     \\ 
% \hline
% \textbf{Chain 6}                & 1                                                                                          & 2                                      & 9                                                                                                                                & 20                                                                                                                                & 360                                                                                                           & 349                                    &                 121                       & 329                                    & 134                                     \\ 
% \hline
% \textbf{Chain 7}                & 0                                                                                          & 2                                      & 8                                                                                                                                & 20                                                                                                                                & 120                                                                                                           & Best-Effort                            &             167                           & Best-Effort                            & 222                                     \\ 
% \hline
% \textbf{Chain 8}                & 0                                                                                          & 4                                      & 26                                                                                                                               & 40                                                                                                                                & 220                                                                                                           & Best-Effort                            &                267                        & Best-Effort                            & 298                                     \\
% \hline
% \end{tabular}
% }

% \caption{Chain configuration and results for case study 1}
% \label{table:case_study_config}
% \end{table}


\subsection{Case Study 1: GPU-enabled Robotic System} \label{sec:case_study}
\noindent\textbf{System Setup.}
This scenario is derived from the PiCAS case study~\cite{choi2021picas}, which is inspired by the F1/10 robotic platform, but introduces additional accelerator segments. %to relevant to the successful accelerated execution of the prescribed processing chains. } 
%The workload is representative of a real multi-process robotic system with several linear and nonlinear chains. This case study was designed to ensure reliable, repeatable, and accurate results. 
The chain configuration of this scenario can be found in Fig.~\ref{fig:case_study}.
There are 8 processing chains, divided into two categories: critical chains (chains 1-6) and non-critical or best-effort chains (BE 1-2). %The chain configurations motivated by an autonomous robotic application can be found in %Table~\ref{table:case_study_config} and are illustrated in Fig.~\ref{fig:case_study}. 
%This case study utilizes a mix of linear and nonlinear chains. As shown in Fig.~\ref{fig:case_study}, chains 1 and 2 are nonlinear and originate from a common initial callback while all other chains are linear. 
Each callback contains one GPU segment with the WCET of 10 ms, i.e., $\forall \tau_i, A_i=10$. %, so, for each chain, the total number of accelerator segments per chain is equal to the number of callbacks in that chain. 
Callbacks have CPU workloads with various execution times, depicted by $E$ in the figure.
%For simplicity of presentation, we configured all accelerator workloads to be identical in duration and type with a worst-case standalone execution time of $10ms$. The chains vary in their total callback length and each callback's CPU-based workload. Every callback within a chain has a variable CPU-based computation requirement, as prescribed by the PiCAS case study on a robotic system, as well as an identical GPU-based workload. 
To compare the maximum end-to-end latency observed from experiments against the worst-case bound from our analysis, we applied the analysis' assumptions to this case study: (i) the PAAM server and its worker threads were pinned to core 0 with real-time priority, and (ii) chain clients were executed by multiple single-threaded executors pinned to other cores. Specifically, the chains were partitioned into four executors, in the same manner as in \cite{choi2021picas}; the executors including critical chains 1-6 were pinned to cores 2-7; the BE chains were assigned to separate executors pinned to cores 2-3 to stress high-criticality chains. BE 1 and 2 are duplicates of chains 1 and 3, respectively. Hence, the BE chains are also periodic, but their response times do not need to be within their periods. 
%We run the critical chains on separate prioritized executors pinned to singular CPU cores $2-7$ in criticality order. The best effort chains are also assigned to separate de-prioritized executors pinned to singular CPU cores 2 and 3 to exaggerate worst-case performance of the highest-criticality chains. The highest-priority critical chain is scheduled to execute on CPU 2 with a periodicity of 120ms, while the lowest-priority critical chain is scheduled to execute on CPU 7 with a periodicity of 360ms. The best-effort chains are also periodic, but their response times are not guaranteed to be within a single period. With this configuration, we are able to analytically upper bound all critical chains response times by applying the analysis in Sec.~\ref{sec:analysis}. %Table~\ref{table:case_study_config} shows the results of the analysis and indicates predictable upper bounds of response time for all critical chains. 


\begin{figure}[t]
	\centering
	\subfloat{
		\includegraphics[width=\linewidth]{figures/rtas-tc6-wc-v2-2-narrow.pdf}
	}
	%	\vspace*{-1mm}
	\caption{Case study 1: Maximum observed chain latency}
	\label{fig:wc_case_study}
\end{figure}
\begin{figure}[t]
	\centering
	\subfloat{
		\includegraphics[width=\linewidth]{figures/rtas-tc-avg-v2-1-narrow.pdf} % ADD THE DISTRIBUTION
	}
	%	\vspace*{-1mm}
	\caption{Case study 1: Chain latency distributions }
	\label{fig:ac_case_study}
\end{figure}

For comparison, we consider the following methods: 
\begin{itemize}
    \item \textbf{ROS~2}: Clients run on the default ROS 2 executors and use the direct invocation method for accelerator access.
    \item \textbf{PiCAS}~\cite{choi2021picas}: Clients execute as in ROS 2, but on the PiCAS executors.
    \item \textbf{PAAM}: Our proposed framework.
    \item \textbf{Analysis}: The worst-case end-to-end latency (response time) computed by our analysis given in Sec.~\ref{sec:analysis}. 
\end{itemize}

\smallskip\noindent\textbf{Results.} 
Fig.~\ref{fig:wc_case_study} compares the maximum chain latency observed from experiments under each method, along with the worst-case latency computed by our analysis. Fig.~\ref{fig:ac_case_study} reports the distributions of observed chain latencies under respective methods. 
%and \ref{fig:ac_case_study} showcase the worst-case and average-case results of our case study when run under 4 contexts. %The first executes PAAM-enabled chains  with a single bucket enabled (i.e. all requests are queued into the same thread-local queue),  the second executes PAAM-enabled chains using multiple buckets that correspond to the 6 CUDA stream priorities supported by the AGX hardware, the third executes PiCAS-enabled chains under the direct-invocation paradigm, and the fourth executes chains under the direct invocation paradigm and with the default ROS2 scheduler (i.e PiCAS-disabled chains). These correspond to the first  four legend items in Fig.~\ref{fig:wc_case_study}; the remaining legend item corresponds to the response time bounds that were calculated using the case study parameters with the PAAM analysis. 
We observed that the maximum observed chain latency under PAAM was always bounded by our theoretical analysis. This observation is juxtaposed with the unbounded response time of the highest-criticality chains without PAAM. In addition, the maximum observed latency of critical chains under PAAM is much shorter than ROS 2 and PiCAS (e.g., more than 50\% reduction for chain 1), which demonstrates the effectiveness of our proposed framework.

%We performed a series of micro-benchmarks on a set of GPU kernels to identify the effect of the PAAM framework on the end-to-end response time of a single kernel launch. The kernels used in this experiment were matrix multiplication, vector addition, histogram generation, and vector reduction. We justify the use of these kernels for micro-benchmarking as they're commonly used in other tasks like DNN inferencing or image processing. In fig.~\ref{fig:microbench} we demonstrate that under ideal conditions, the round-trip execution time of kernels with the PAAM server is only marginally longer than those kernels under the direct invocation model even though PAAM introduces some additional communication and scheduling delay. 



\subsection{Case Study 2: Autoware Reference System w/ GPU \& TPU}
% \begin{figure}[h] 
% 	\subfloat{
% 		\includegraphics[width=1\linewidth]{figures/autoware_chain.pdf}
% 	}
% 	\caption{Chain configuration of Apex.AI's Autoware reference system~\cite{web:ros2refsys}{\red (It'd be nice to redraw this figure by adding executors, nodes, and callbacks so that it can replace the original chain example} {\blue The callback to executor allocation is different for each of the case study scenarios on the reference system. The first config is 4 singlethreaded executors with some callbacks added to each. Then there is the multithreaded case where all callbacks belong to the same executor. }}
%     \label{fig:autoware_model}
% \end{figure}

\noindent\textbf{System Setup.}
To evaluate the benefit of PAAM in a more complex scenario, we used the Apex.AI's Autoware reference system~\cite{web:ros2refsys}. The system resembles the lidar-based perception pipeline of Autoware.Auto~\cite{web:autowareauto}, as illustrated in Fig.~\ref{fig:autoware_model}. We augmented this system by incorporating GPU and TPU segments into every callback, excluding the seven dedicated to the behavior planner to prevent accelerator overload. Recall that the Coral TPU does not allow for more than one context to exist at a time; so, to fairly evaluate the impact of PAAM on the reference system, we assigned a TPU inferencing workload to the single rear lidar points transformer callback. This setup permitted a straightforward comparison between the PAAM and direct invocation methods, with the latter requiring only one TPU context.
%\hyoseung{Accelerator segments were added to all callbacks or some of them?}\daniel{all callbacks except for behavior planner node} 
The reference system produces several Key Performance Indicators (KPIs):

%\smallskip\noindent\textbf{Key performance indicators (KPIs).}  The Autoware reference system records and evaluates several key performance indicators including:
\begin{itemize}
    \item {\bf Hot Path Latency}: The hot path, outlined in Fig.~\ref{fig:autoware_model}, is composed of the chain of callbacks from the lidar sensor to the collision estimator. This is the most critical chain in the system as it indicates the time to react to obstacles. %A lower latency of this path indicates better system performance. 
    \item {\bf Behavior Planner Period}: The behavior planner is set to execute with a period of 100 ms. If the execution is blocked, the actual period may be prolonged. Lower variations in the measured period from the planner period are better.
    \item {\bf Hot Path Message Drops}: Dropped hot path messages show how many callbacks in the hot path missed their input messages in the current instance of the chain. A lesser amount of dropped messages indicates better performance. 
\end{itemize}

Unlike the first case study, we evaluate each method with both single-threaded (ST) and multi-threaded (MT) executors. 
%\noindent\textbf{Autoware Reference System Configuration:}
%To thoroughly evaluate the impact of PAAM on the performance of the accelerator-enabled \emph{Autoware reference system}, we set up experiments in the following manner. 
%Similar to all the other case studies, the PAAM server and all worker threads are bound to CPUs 0 and 1. 
%We evaluated the accelerator-enabled Autoware reference system with two different executor configurations:
\begin{itemize}
    %\item \textbf{Single-threaded Executor:} We evaluated PAAM against the direct invocation approach where all nodes are assigned to a singular single-threaded executor using both the default ROS 2 callback scheduler and the PiCAS callback scheduler.
    \item \textbf{4$\times$ST:} We partitioned the reference system workload to four ST executors, each pinned to a separate CPU core. 
    %For this experiment, we configured the Autoware reference system to run on four separate single-threaded executors, pinned to separate CPU cores. We evaluated the performance of the Autoware reference system under three scenarios. The first scenario creates four default ROS 2 executors to run the reference system and uses direct invocation for accelerator workloads. The second scenario creates four PiCAS executors to run the reference system and also uses direct invocation for accelerator workloads. The final scenario creates four PiCAS executors to run the reference system and uses PAAM for accelerator workloads. 
    \item \textbf{MT:} The system runs in one MT executor. To use the same number of cores as 4$\times$ST, we configured the number of threads to 4 and pinned the threads to to 4 cores.
    %For this experiment, we configured the Autoware reference system to run on a single multi-threaded executor pinned to 4 CPU cores (2-5) and duplicated the scenarios from the previous experiment. 
\end{itemize}

\noindent\textbf{Results.} Fig.~\ref{fig:autoware_latency} depicts the end-to-end latency of the hot path across all system configurations. Overall, PAAM outperformed the rest, with PiCAS coming in second and ROS 2 trailing behind.
Focusing on the 4$\times$ST case, the priority-based chain scheduling of PiCAS achieves a 68\% reduction in the maximum hot path latency over ROS~2, decreasing from 510~ms to 163~ms. On top of this, PAAM further reduces the latency by 51\% compared to PiCAS, bringing it down to 79~ms. The substantial improvement by PAAM can be attributed to its ability to handle numerous low-criticality chains competing for accelerators in the reference system. The MT case follows the same trend, but interestingly, all three methods maintain poorer worst-case performance than in the ST$\times$4 case. This is because, with ST, the hot path encounters less blocking from low-criticality chains.

%We observed a reduction in end-to-end latency from ROS 2 to PiCAS. In this case, the maximum observed latency was reduced by $83\%$ from $1497ms$ to $250ms$. When switching from the direct-invocation approach with PiCAS to the PAAM approach with PiCAS, we observed an additional reduction in the maximum observed latency of $40\%$ from $250ms$ to $150 ms$. In the singlethreaded case, we found the same trend. We observed a reduction in end-to-end latency from the direct invocation approach running on the ROS 2 executor to that approach running on the PiCAS executor. In this case, the maximum observed latency was reduced by $87\%$ from $1331ms$ to $165ms$. Furthermore, when switching from the direct invocation approach to PAAM's approach, we observed an additional reduction in latency of $55\%$ from $165ms$ to $73ms$. 

Figs.~\ref{fig:autoware_period} and \ref{fig:autoware_drops} show the observed distribution of behavior planner period and the number of dropped messages per hot path instance, respectively. PAAM achieves much lower variations from the preset 100 ms period, while simultaneously ensuring no message drops. From all these results, we conclude that PAAM can yield a significant improvement over the state-of-the-art, especially in a complex robotic environment.

%In Fig.~\ref{fig:autoware_period}, we show the observed distribution of behavior planner period under all system configurations. For this test, a lower variation from the preset $100ms$ period of the behavior planner indicates better performance. When running the autoware reference system with the default multithreaded executor and using direct invocation, we observe that our measured period variations are greater than $140ms$. Switching from the default ROS 2 multithreaded executor to the PiCAS multithreaded executor reduces the behavior planner period variations from $140ms$ to $30ms$. Changing from the direct-invocation approach to the PAAM approach, we observed a further reduction in behavior planner period variation from $30ms$ to $15ms$. When running this case with four singlethreaded executors, we observe a similar trend. When using this configuration with the ROS 2 default executor and direct invocation, we notice maximum period variations of up to $100ms$. When using the PiCAS executor and direct invocation, we observe variations that are less than $1ms$. Furthermore, using this executor configuration with PAAM maintains a planner period variation of less than $1ms$. 


%\noindent\textbf{Hot path drops:} In fig.~\ref{fig:autoware_drops}, we show the number of dropped messages per hot path instance under all system configurations. Ideally, we should not drop any messages on the hot path. When running the autoware reference system with the ROS 2 default multithreaded executor and direct invocation, we see that the hot path counted up to four dropped messages per hot path instance. In the case of the PiCAS executor and direct invocation, we observe a maximum of one dropped message per hot path instance. When running the autoware reference system with the PiCAS executor and PAAM, we observe a maximum of zero dropped messages per hot path instance. In the case of four singlethreaded executors, we observe a similar trend. With the default ROS 2 executor and direct invocation, we observe a maximum of three dropped messages per hot path instance. Moreover, using the PiCAS executor and direct invocation, we observe a maximum of one dropped message per hot path instance. When using the PiCAS executor and PAAM, we observe no dropped messages per hot path instance.  

%{\magenta Since the USB TPU accelerator does not support more than one simultaneous execution context, we are only able to evaluate the performance of the TPU under PAAM and \emph{not} under direct invocation. For these cases, the TPU workload consists of identifying, boxing, and labeling objects within images. We used Inception v2\cite{DBLP:journals/corr/IoffeS15} with an isolated WCET of 24ms.}{\red (Copied from TPU subsection; needs to be edited)}

\begin{figure}[t]
	\centering        
 	\subfloat[Hot Path Latency]{\label{fig:autoware_latency}            
		\includegraphics[width=.98\linewidth]{figures/autoware_latency.pdf}
	}\\
	\subfloat[Behavior Planner Period]{\label{fig:autoware_period}
		\includegraphics[width=.48\linewidth]{figures/bh_period.pdf}
	}        
        \subfloat[Hot Path Drops]{\label{fig:autoware_drops}
		\includegraphics[width=.48\linewidth]{figures/autoware_drops.pdf}
	}
	%	\vspace*{-1mm}
	\caption{Case Study 2: Autoware reference system results}
	\label{fig:autoware_results}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	\subfloat{
% 		\includegraphics[width=\linewidth]{figures/hp_drops.pdf}
% 	}
% 	%	\vspace*{-1mm}
% 	\caption{Hot Path Drops}
% 	\label{fig:autoware_drops}
% \end{figure}

%\subsubsection{Single-threaded Executor}
%For this experiment, PAAM was evaluated when running the Autoware reference system configured so that every callback is scheduled and executed by a lone single-threaded executor. In figure~\ref{fig:autoware_single}, we show the key performance metrics of the reference system in four scenarios. In the first scenario, both PiCAS callback scheduling and PAAM are disabled; each accelerator-enabled callback executes the accelerator workload via the direct invocation approach. For the second scenario, we enable PAAM for accelerators, but disable PiCAS callback scheduling; this is used to directly compare with the previous case. The third scenario enables PiCAS and disables PAAM. The fourth scenario enables both PiCAS for prioritized callback scheduling and PAAM for prioritized accelerator segment scheduling. In the PiCAS-enabled scenarios, PAAM outperforms the direct invocation approach by facilitating an $83\%$ reduction in the end-to-end response time of the hot path. In the PiCAS-disabled scenarios, PAAM reduces end-to-end hot path latency by \daniel{TODO: add}

%\subsubsection{4 Single-threaded Executors}


%\subsubsection{Multi-threaded Executor}


\subsection{PAAM Overhead Analysis}\label{sec:ovh_brkdn}
	
\noindent\textbf{Overhead Breakdown.}
%In our pursuit to comprehensively understand the effects of PAAM on the response time of critical callback chains, we conducted an exhaustive study cataloging the various causes of overhead incurred when utilizing PAAM. 
We sought to unpack the overhead associated with PAAM's servicing of client requests, in the context of best, average, and worst-case scenarios. As shown in Figure~\ref{fig:breakdown}, the overhead arising from PAAM's utilization spans from 198 $\mu$s in the optimal scenario to 391 $\mu$s in the most unfavorable one. 
A careful analysis reveals that a significant portion of the time is consumed by the DDS transport, sending a request message to the server in the control plane. The Iceoryx-enabled Cyclone DDS that the PAAM implementation uses is reported to have a latency of only a few $\mu$s for 1 KB payload~\cite{web:iceoryx_latency}~\cite{web:TSC-RMW-Reports}, which is much smaller than our control-plane message size (72 B). However, we found that its latency increases significantly when integrated into the ROS 2 ecosystem due to additional interface layers. This result further reinforces the rationale behind our design choice to have a separate data plane. Interestingly, we found that PAAM's request queueing, worker awakening, and scheduling, consume the least amount of time. 
%A careful analysis reveals that a significant portion of the time is consumed during the phases of request generation, transmission, and notifying clients of kernel completion when PAAM is engaged. The delay in message creation is tied to the dynamic memory allocation for the message object, and the process involved in filling out the message data structure. 
%The transmission delay is largely due to the DDS-related latency inherent in Inter-Process Communication (IPC) and message transport. 
%The messages are of fixed size and are transmitted using zero-copy with Iceoryx-enabled Cyclone DDS. The client waking component of the server overhead imposes a moderate impact on the total overhead. We can attribute this delay to locking and condition variable usage in shared memory. Interestingly, we found that request queueing, worker awakening, and scheduling consume the least amount of time. In the average case, the request queueing takes less than $1\mu s$ whereas we observe $4\mu s$ of queueing delay in the worst case. Furthermore, the worker awakening consumes an average of $23\mu s$ and a maximum of $51\mu s$; this delay can also be traced back to the locking and condition variable usage.

%Interestingly, we found that the awakening of worker threads - leveraging pthread implementations of condition variables - consumes the least amount of time. Furthermore, we noticed a moderate delay in popping requests from thread-local queues and any delays are primarily attributable to locking mechanisms necessary to protect thread-shared server data structures and the inherent latency of using the standard library implementation of priority queues.
%The process of awakening client threads from sleep imposes only moderate delay. Any delay that does occur in this context can be traced back to the locking and condition variable usage in shared memory.

\smallskip\noindent\textbf{GPU Preemption Delay with Multiple Buckets.}
Since our framework leverages a multi-bucket approach with preemptive execution for supported accelerators, we measured the GPU preemption delay that is incurred when executing a kernel on a high-priority stream while a low-priority stream is also executing a kernel. For this benchmark, as shown in Table~\ref{table:pd}, we observed that the maximum incurred preemption delay was $142\mu s$ and the average preemption delay was $95.3\mu s$.

% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Mean   & Max    & Stddev \\ \hline
% 95.300 & 142.33 & 10.735    \\ \hline
% \end{tabular}
% \caption{GPU bucket\\preemption cost ($\mu$s)}
% \label{table:pd}
% \end{table}

%{ In order to further evaluate the impact of PAAM on the response time of critical callback chains, we conducted a study to break down the overhead of PAAM. Figure~\ref{fig:breakdown} shows the breakdown of the overhead incurred by using PAAM in the best, average, and worst cases. In the best case, the overhead is 1.018ms, and in the worst case, the overhead is 1.395ms. The biggest time consumers of using PAAM are the request generation, request transmission, and the request queueing stages. The delays in message generation can be attributed to dynamic memory allocation of the message object as well as populating the message data structure. The message transmission delay can be attributed to the DDS-related delays for IPC and message transport. The queueing delays can be attributed to locking mechanisms used to protect server data structures and dynamic memory allocation/population mechanisms required for worker threads to execute requested workloads. Worker thread waking takes the shortest amount of time and threads are awakened by leveraging the pthread implementations of condition variables. Delays incurred from popping the requests from the thread-local queues can be attributed to locking mechanisms necessary to protect thread-shared server data structures and standard popping delay from using std::priority_queue mechanisms. Waking the client threads from sleep, interestingly, does not incur tremendous delay and can all be attributed to delays in locking and condition variable usage in shared memory. }
\begin{figure}[t]
	\centering
	\subfloat{
		\includegraphics[width=\linewidth]{figures/overhead.pdf}
	}
	%	\vspace*{-1mm}
	\caption{Overhead breakdown}
	\label{fig:breakdown}
\end{figure}
%\subsubsection{Blocking Time Comparison}

\smallskip\noindent\textbf{Kernel Response Time.}
To assess the impact of overhead in kernel execution, we report the response time of several well-known GPU benchmark kernels when each runs alone in the system. The results are depicted in Figure~\ref{fig:microbench}. The round-trip execution time of kernels with the PAAM server is only slightly longer compared to kernels that are directly invoked without the framework. We consider such a small increase in kernel response time acceptable given the huge benefit achievable by our framework. 
%In order to evaluate the impact of our PAAM framework on the response time of GPU kernels, we conducted a thorough set of micro-benchmarks using commonly utilized kernels such as matrix multiplication, vector addition, histogram generation, and vector reduction. These kernels were chosen due to their frequent usage in various tasks including DNN inferencing and image processing. Through our evaluation, we demonstrate that even under ideal conditions, the round-trip execution time of kernels with the PAAM server is only slightly longer compared to kernels that are directly invoked without the framework. This is despite the fact that PAAM introduces additional communication and scheduling delays. In Figure~\ref{fig:microbench}, we present the results of our benchmarks, which clearly show the negligible impact of PAAM on kernel response time. Our findings highlight the effectiveness of PAAM in providing predictable real-time support for accelerators without adversely affecting performance, making it a promising framework for modern autonomous systems
\begin{table}
    \begin{minipage}{0.58\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/microbenchmarking.pdf}
        \vspace{-8mm}
        \captionof{figure}{Kernel response time}
	\label{fig:microbench}
    \end{minipage}\hfill
    \begin{minipage}{0.38\linewidth}
        \centering
        \begin{tabular}{|c|r|}
        \hline
        Results & Time ($\mu$s)\\\hline
        Mean   & 95.30 \\ \hline
        Max    & 142.33 \\ \hline
        Stddev & 10.74    \\ \hline
        \end{tabular}
        \caption{GPU bucket preemption cost}
        \label{table:pd}
    \end{minipage}
\end{table}

% \begin{figure}[t]
% 	\centering
% 	\subfloat{
% 		\includegraphics[width=.6\linewidth]{figures/microbenchmarking.pdf}
% 	}
% 	%	\vspace*{-1mm}
% 	\caption{Worst Case Execution Time of Kernel}
% 	\label{fig:microbench}
% \end{figure}

\subsection{Analytical Study} \label{rand_chain}
To explore the performance characteristics of our analysis, we conduct two experiments that examine the schedulability of chainsets based on varying parameters: the number of chains in a chainset and the accelerator-to-CPU utilization ratios. 

For the first experiment, we established a fixed chain length of 4 callbacks per chain for a system with one accelerator. We then executed 1,000 schedulability tests for each distinct number of chains per chainset. The chains generated had random periodicity, but we ensured a strict 1:1 Accelerator:CPU utilization ratio per period, with the total utilization equally distributed amongst all the callbacks within the chain. Figure~\ref{fig:vc} shows the results, conducted with a varying number of chains per chainset. %We also present the outcomes of the schedulability tests performed with different utilization per chain within each chainset. As predicted, the schedulability of chainsets experiences a decline as the number of chains within a chainset increases, and also diminishes with higher total utilization per chain.

The second experiment was designed in a similar manner, but 
%with a fixed configuration of 4 chains per chainset and 4 callbacks per chain. Utilizing this setup, we evaluated the schedulability of 1000 randomly constructed chainsets with preset CPU-time:GPU-time ratios. 
the ratio of accelerator utilization to CPU utilization per chain was varied from 1:9 to 7:3. The results of these schedulability tests are illustrated in Figure~\ref{fig:vr}. Interestingly, even when the utilization per chain remains constant, the schedulability of a chainset decreases as the accelerator-to-CPU utilization ratio escalates. This can be attributed to the contention on the singular accelerator that all chains and callbacks share. \par

%To analyze the characteristics of our admissions control, we performed two studies that characterized the schedulability of chainsets with varying numbers of chains per chainset, varying chain utilization, and varying CPU-time to GPU-time ratios. For the first experiment, we fixed a reasonable chain length of 4 callbacks per chain and performed 1000 schedulability tests for each number of chains per chainset. We generated chains with random periodicity, but maintained a strict 1:1 ratio of CPU:GPU utilization per period and divided the total utilization evenly among all the callbacks in the chain.  In figure~\ref{fig:vc} we show the results of our schedulability tests with a varying number of chains per chainset. We also show the schedulability tests performed with varying utilization per chain in each chainset. As expected, the schedulability of chainsets decreases as the number of chains in a chainset increases and also decreases with a larger total utilization per chain.\par For the second experiment, we fixed our chainsets to have 4 chains per chainset and 4 callbacks per chain. With this, we tested the schedulability of 1000 randomly generated chainsets with a fixed CPU-time:GPU-time ratios. We then varied the combined CPU and GPU utilization per chain from 10\% to 70\%. In figure~\ref{fig:vr}, we show the results of those schedulability tests. Even with the same utilization per chain, the schedulability of a chainset decreases as the ratio of GPU-time to CPU-time increases. This can be attributed to there being a single accelerator that all chains and callbacks are sharing. \par


\begin{figure}[t]
	\centering
        \subfloat[\# of chains per chainset]{\label{fig:vc}\includegraphics[width=0.48\linewidth]{figures/rtas-vc.pdf}}     
  	\subfloat[Accelerator util. : CPU util.]{\label{fig:vr}\includegraphics[width=0.48\linewidth]{figures/rtas-vr.pdf}}   
	%	\vspace*{-1mm}
	\caption{(a) Schedulability of Chainsets with a Varying Number of Chains per Chainset (b) Schedulability of Chainsets with Variable CPU-time to accelerator-time Ratios}
	\label{fig:vcr}
\end{figure}
% \begin{figure}[t]
% 	\centering
% 	\subfloat{
% 		\includegraphics[width=0.4\linewidth]{figures/rtas-vr.eps}
% 	}
% 	%	\vspace*{-1mm}
% 	\caption{Schedulability of Chainsets with Variable CPU-time to GPU-time Ratios {\red (make the font size, width, height same as fig.~\ref{fig:vc})}}
% 	\label{fig:vr}
% \end{figure}
\begin{figure}[t]
    \centering
    	\subfloat{
 		\includegraphics[width=0.98\linewidth]{figures/tc_hm_distr.pdf}
 	    }
        \caption{ Case Study 3: Chain latency distribution}
 	\label{fig:wc_case_study2tpu}
\end{figure}
\begin{figure}[t]
	\centering
 	\subfloat{
 		\includegraphics[width=0.98\linewidth]{figures/tc_hm_wc.pdf}
        } 
        \caption{  Case Study 3: Maximum observed chain latency }

 	%	\vspace*{-1mm}
 	\label{fig:ac_case_study2tpu}
 \end{figure}

 \subsection{Case Study 3: Overloaded GPU} \label{sec:case_study}

 %\smallskip\noindent\textbf{Test Case 2: } 
 The primary goal of this case study was to demonstrate the effectiveness of our PAAM framework in ensuring worst-case response time guarantees for GPU-enabled critical callback chains even under overloaded conditions. To accomplish this, we executed six callback chains divided into two categories - two critical chains and four best-effort chains. The two critical chains were schedulable under PAAM analysis, with bounded execution time. Chain 1, with the highest priority, had a $120ms$ period and a GPU-dominated workload with a standalone worst-case execution time of $52ms$. Chain 2, with the second-highest priority, had a period of $220ms$ with the same GPU-dominated workload. Chains 3-6 were best-effort chains executing continuous back-to-back GPU-dominated workloads of $52ms$ each.

% \begin{table}[t]
%  \resizebox{\linewidth}{!}{%
% %\resizebox{.95\textwidth}{!}{%
%  \begin{tabular}{|l|l|l|l|l|l|l|l|}
%  \hline
%  \textbf{Chain}   & \textbf{Chain Priority} &\textbf{\# Callbacks} & \textbf{\begin{tabular}[c]{@{}l@{}}Total CPU-time\\ (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Total GPU-time \\ (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Period\\ (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Bounded \\ Response \\ Time\\ (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Observed \\ Response\\ Time\\ (ms)\end{tabular}} \\ \hline
%  \textbf{Chain 1} & \textbf{6} & \textbf{1} & \textbf{2} & \textbf{52} & \textbf{120}  & \textbf{106} & \textbf{95}           \\ \hline
%  \textbf{Chain 2} & \textbf{5} & \textbf{1} & \textbf{2} & \textbf{52} & \textbf{220} & \textbf{210} & \textbf{138}           \\ \hline
%  \textbf{Chain 3} & \textbf{0} & \textbf{1}  & \textbf{2} & \textbf{52}  & \textbf{N/A} & \textbf{Best Effort} & \textbf{332}        \\ \hline
%  \textbf{Chain 4} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{52} & \textbf{N/A} & \textbf{Best Effort}  & \textbf{330}         \\ \hline
%  \textbf{Chain 5} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{52} & \textbf{N/A} & \textbf{Best Effort} & \textbf{328}          \\ \hline
%  \textbf{Chain 6} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{52} & \textbf{N/A} & \textbf{Best Effort} & \textbf{335}          \\ \hline
%  \end{tabular}%
%  }
%  \caption{Chain Configuration for Case Study 2}
% \label{table:case_study_2_config}
% \end{table}

In Figure~\ref{fig:wc_case_study2tpu}, and Figure~\ref{fig:ac_case_study2tpu}, we present the results of our test case, which indicate that our framework provides bounded worst-case response times for critical chains as well as competitive average-case performance for best-effort chains. We performed the execution of chains in three contexts: PAAM-enabled chains, PiCAS-enabled chains with direct invocation, and chains executed by the default ROS 2 scheduler with direct invocation. In both direct invocation cases, we observed that the worst-case response times of critical chains were similar to that of best-effort chains since access to the accelerator was not determined by chain priority. Without PAAM, the GPU became overloaded with requests and resorted to its driver-inherent scheduling. However, for critical chains under PAAM, we observed a dramatic reduction in worst-case response times due to regulated and priority-driven accelerator access. blue For the highest criticality chain, we observed a 60\% reduction in response time when accelerator requests were scheduled under PAAM compared to the accelerator driver inherent fairness-based scheduling seen under the direct-invocation model. For the lower-priority critical chain, we also observed a 45\% reduction in response time, while the response time for the non-critical best-effort chains increased an average of 29\%. The response time increases, in the worst case, are expected, as the goal of PAAM is to guarantee the response time of critical chains at the expense of best-effort chain response time.  We also observed a decline in average-case throughput and an increase in worst-case response time for best-effort chains. At the same time, we observed a  79\% decrease in the average case response time {of the highest criticality chain and a bounded worst-case response time for all critical chains. We also observed a 74\% reduction in the average case response time for the lower-priority critical chain. Also, in the average case, the response time of all other PAAM-enabled best-effort chains is roughly the same as, if not marginally better, than those run without PAAM. Despite the additional overhead incurred by using PAAM, we can attribute the similar performance to the lack of GPU context switching delays incurred under the direct invocation model - as the PAAM server process only necessitates a single CUDA context. Our findings demonstrate the effectiveness of PAAM in providing predictable and analyzable real-time support for GPU-enabled critical chains, even under overloaded conditions, making it a valuable tool for modern autonomous systems.

%This case study was designed to showcase the PAAM framework's ability to guarantee the worst-case response time of GPU-enabled critical callback chains despite overloaded conditions. This test involves the execution of 6 callback chains, divided into the same two categories as before: with 2 critical chains and 4 best-effort chains. The 2 critical chains are schedulable under PAAM analysis with bounded execution time. 

%Chain 1, the highest priority chain, executes with a $120ms$ period and has a GPU-kernel dominated workload whose standalone worst-case execution time is $52ms$. Chain 2, with the second highest chain priority, executes with a period of $220ms$ with the same $52ms$ GPU-dominated workload. Chains 3-6 are best effort chains that execute continuous back-to-back GPU-dominated $52ms$ workloads. Under these conditions, without PAAM, the GPU becomes overloaded with requests and resorts to its driver-inherent scheduling. However, with PAAM-enabled clients, we observe a decline in average-case throughput and an increase in worst-case response-time of best-effort chains. At the same time, we observe a decrease in average-case response-time and a bounded worst-case response-time of critical chains. 

%In Fig.~\ref{fig:wc_case_study2}, we show that the results from this test case indicate that our framework provides bounded worst-case response times of critical chains. We do this by executing the chains in three contexts: with PAAM and PiCAS-enabled chains, with direct invocation and PiCAS-enabled chains, with direct-invocation and PiCAS-disabled chains. For both direct invocation cases, we observe that the worst-case response times of critical chains is similar to that of the best-effort chains, since the access to accelerator is not determined by chain priority. However, for the critical chains under PAAM, we observe dramatically reduced and analytically bounded worst-case response times as a result of regulated and priority-driven accelerator access.    
 
 \subsection{Case Study 4: Overloaded TPU } \label{sec:case_study_TPU}
 To showcase the effectiveness of our framework with multiple types of accelerators, we duplicated case study 2 and applied it to the Coral USB TPU accelerator. Since the USB TPU accelerator does not support more than one simultaneous execution context, we are only able to evaluate the performance of the TPU under PAAM and \emph{not} under direct invocation. For these cases, the TPU workload consists of identifying, boxing, and labeling objects within images. We used Inception v2\cite{DBLP:journals/corr/IoffeS15} with an isolated WCET of 24ms.
 
  \noindent \textbf{Test Case 1:} The primary goal of this case study was to demonstrate the effectiveness of our PAAM framework in ensuring worst-case response time guarantees for TPU-enabled critical callback chains even under overloaded conditions. To accomplish this, we executed six callback chains divided into two categories - two critical chains and four best-effort chains. The two critical chains were schedulable under PAAM analysis, with bounded execution time. As seen in Fig.~\ref{fig:tpu} shows the results of this test case, and demonstrates PAAM's ability to coordinate and bound the worst-case response times of critical chains, even when using a TPU accelerator. In Fig.~\ref{fig:tpu_dist}, we also show the distribution of end-to-end response time of all of the chains using the TPU via PAAM.  

 \begin{figure}[t]
 	\centering
 	\subfloat{
 		\includegraphics[width=0.98\linewidth]{figures/tc_2_tpu_wc.pdf}
 	}
 	%	\vspace*{-1mm}
 	\caption{Case Study 4: Maximum observed chain latency}
 	\label{fig:tpu}
 \end{figure}
 \begin{figure}[t]
 	\centering
 	\subfloat{
 		\includegraphics[width=0.98\linewidth]{figures/tc_2_tpu_distr.pdf}
 	}
 	%	\vspace*{-1mm}
 	\caption{Case Study 4: Chain latency distribution}
 	\label{fig:tpu_dist}
 \end{figure}

 


==> draft/6-Example.tex <==
\subsection{Example with GPU Kernel Request}
To provide an example of the exact execution flow of the client and AAMF server, we will discuss a simple ROS 2 client callback that needs to execute a simple floating-point matrix multiplication kernel on a GPU. Upon server and client initialization, we require that both already know the appropriate request and response data structures needed to ensure the client can transport data to the server without any copy operations in shared memory. Specifically when the server initializes, it polls GPU hardware information about stream priority levels, and creates buckets that correspond to each stream priority. In the case of a discrete GPU such as the Nvidia Geforce GTX 1080ti or an integrated GPU such as the Volta architecture iGPU on the Nvidia Jetson AGX Xavier, the there are 6 supported CUDA stream priorities; priority level $-5$ is the highest, and priority level $0$ is the lowest. Once the system has determined the amount of available stream priorities, our GPU initializer will create 6 streams, one for each priority and store their pointers in an array for use at a later time. After the streams are initialized, the AAMF server executor will create the buckets by assigning each prioritized CUDA stream to a standalone worker thread. These threads immediately suspend as their job queues are empty. At this point, initial server configuration is complete and the executor spins, awaiting registration from client nodes. At this point, if un-registered nodes request accelerator resources, their requests will be immediately rejected. \par
During client initialization, the first task is to register with the AAMF server. This process is straightforward and simply requires encapsulating information about the client executor process, the callback identifier, anticipated kernels, and callback chain priority. In this example we assume that the client anticipates  needing 1 kernel, the matrix multiplication kernel. This information is then sent to the server over the standard ROS 2 DDS. Upon receiving the request from the client, the AAMF server will log important callback metadata, will assign a bucket to the callback based on a simple heuristic, and will match the anticipated kernels with request-response data types and allocate those in shared memory. So, for this example, let us also assume that the client specifies the maximum chain priority in the system upon registration -- the bucket assignment will correspond to the maximum priority CUDA stream. The server will then encapsulate maps of the kernel to shared memory ID and send them back to the client in the handshake response. Once the client receives the handshake response, it stores the association between kernel type and shared memory ID for later usage. \par

\begin{figure}[t]
	\centering
	\subfloat{
		\includegraphics[width=0.75\linewidth]{figures/Example.pdf}
	}
	%	\vspace*{-1mm}
	\caption{Example Client Request for GEMM Kernel}
	\label{fig:example}
\end{figure}
Let us assume, for this example, that the callback necessitating the GPU matrix-multiplication kernel, is the producer of input data and is triggered by a timer. Once the timer triggers the callback to launch on the executor, the process can attach to the shared memory region specified by the server for the specific kernel that it needs AAMF to execute. Then, the client will invoke the AAMF synchronous wrapper to populate data structures, send an access request, and wait for completion. The wrapper forces the client to directly write input matrices to shared memory as shown in Fig.~\ref{fig:sync_wrapper}. Subsequently, the client waits for notification from the server that the result is ready and in shared memory. On the server side, the shared memory regions are always attached to the AAMF executor process. When it receives an access request from a client and assigns it into the appropriate bucket, the request is then sorted by priority in the thread-local queue. Once an item is in the queue and if the bucket was previously sleeping, the AAMF server request callback will wake up the bucket. Upon notification, the bucket will pop the highest priority request from the job queue and determine which kernel needs to be executed. Then, the specific GPU kernel wrapper is invoked and passes a smart pointer to the previously attached shared memory region for the requested kernel to directly invoke the kernel operation on the data in shared memory. At this time, the bucket will also pass a parameter to the kernel wrapper that identifies which CUDA stream to execute the kernel on.  \par
When executing the kernel, if the server is using a unified memory model with an integrated GPU (iGPU), there are no memory copies of input matrices from host to device, or from device to host. The input matrices are used directly by iGPU execution units and the results are directly written into shared memory. For server instances that are associated with discrete GPUs, input and output matrix memory-copy operations are facilitated through device driver APIs and direct-memory-access (DMA).  At kernel execution completion, the server will notify the client in shared memory either through updating a status variable or waking the client executor process with a conditional variable. Once the client receives the notification that the server has completed the execution of the kernel, the result is directly accessible in shared memory as shown in Fig.~\ref{fig:sync_wrapper} and can be directly published to a topic, or can be used by the requesting callback for any other purpose.\par 
At this point, the client callback does not need to exit. If more than one matrix multiplication is needed on different sets of data, the client can rewrite to the pre-existing shared memory regions and submit more requests to the AAMF server. However, this is not a requirement. The client callback can exit and be triggered again at a later time by the timer without having to re-register with the AAMF server. In fact, it can directly write to the previously used shared memory regions without any data conflicts. 

==> draft/revision_letter.tex <==
\newpage
\appendix

\begin{center}
\Large \textbf{Revision Letter}
\end{center}
%\vspace{-1mm}
We would like to thank all the reviewers for the time and effort in reviewing our manuscript, and we truly appreciate the constructive comments. We have made changes accordingly throughout the manuscript, including significant additions in approach details and experiments.
\vspace{-2mm}
\section{Changes}
All major changes in this revision are highlighted in blue in the manuscript. 
Here, we summarize the changes, and use \textbf{[R\#]} to denote that the change is related to the reviews from reviewer \#.

In Sec.~\ref{sec:sys_model}, we modified our system model to include additional parameters to consider multiple accelerator segments per callback and to clarify our linear chain model.  \textbf{[R1]} 

In Sec.~\ref{rel_work_rtas} we added a discussion and consideration of the work presented in \cite{Casini_2022_het}.\textbf{[R1]} 

In Sec.~\ref{sec:client_reg}, we added an additional figure outlining the server data structure that maintains and keeps track of client callbacks, shared memory regions, and other information. We also significantly expanded our discussion of the server data structures and clarified the process by which the runtime monitor checks the status of clients and garbage-collects wasted memory. \textbf{[R2]}

In Sec.~\ref{sec:data_trans} we added a figure describing a sample shared memory region and pointed out the mechanisms used for data transport and client wakeup. Also, in Sec.~\ref{flows} explain the potential advantages of using the asynchronous AAMF wrapper when making requests. We also added detail explaining how we were able to wake up client threads using shared memory and how the synchronous wrapper forces clients to busy-wait on a shared-memory status variable. We also provided more detail about how AAMF handles request cancellations and addressed the data consistency concern. Furthermore, in Sec.~\ref{gpu_consid}, we explained how third-party libraries are supported by AAMF.  \textbf{[R1, R2]} 

In Sec.\ref{sec:analysis}, we made significant changes to clarify the proposed analysis approach and to improve the presentation and proof details. First, we extended our analysis to consider multiple buckets such that it matches the GPU implementation of AAMF.\textbf{[R1, R3, R4]}.
Second, we added Lemma~\ref{lm:req_arrival} with proof to clarify how ``+1'' captures the carry-in effect and why it is safe.\textbf{[R1, R3]} Third, we added a list of AAMF behavior rules to help follow analysis details and to clarify how preemption among worker threads and non-preemptive execution within each worker thread work.\textbf{[R1, R3]}. Fourth, we reorganized equations with the new notation to improve the presentation quality.\textbf{[R1, R3]}. Fifth, we rewrote the WCRT analysis and its proof (Theorem~\ref{lm:wcrt_task}) by introducing the existing analysis and the reasoning behind the additional interference we considered. \textbf{[R3]}. Lastly, we explained how the WCET of a GPU segment estimated in isolation can be used and what overhead to consider at the end of this subsection.\textbf{[R3, R4]}

In Sec.~\ref{sec:eval} we clarified the design on the robotic system and mentioned testing parameters. Furthermore, in Sec.~\ref{sec:case_study}, we reran our experiments to showcase both single- and multi-bucket request execution in accordance with the analysis. We introduced 2 new figures explained, in more detail, the chain configuration we used in the case study. We also added a table that explained the setup details behind and the results of the second case study. \textbf{[R1, R2]}

In Sec.~\ref{sec:ovh_brkdn}, we added an additional figure and provided analysis of the overhead incurred by using the AAMF framework (incl. communication cost, server queueing delay, etc.). \textbf{[R1, R2, R3]}
\section{Response to questions and comments}

Besides the comments and questions that are addressed in the above changes list, in the following, we answer some other questions and comments from the review.

\smallskip
\noindent
\textbf{Review \#1:}
%\emph{\blue R1.1. "what is the "direct invocation” model?" } The direct invocation model is a programming paradigm where shared accelerators are directly invoked by callbacks without any underlying coordination, management, or consideration for chain priorities. 
\emph{\blue R1.1. "it could be useful to discuss how the result of Lemma 2 can be worse (i.e., bigger) than the sum of the results (for each callback in a chain) for Lemma 1"} We added a discussion below Lemma~\ref{lm:max_waiting2} about when each approach may outperform the other.

\emph{\blue R1.2. "Page 15, line 721: Is this robotic application derived from some other work, or has the data been invented for this specific paper?" }  This scenario was directly derived from the PiCAS case study, which is inspired by the F1/10 vehicle platform, but introduces additional GPU-based segments relevant to the successful accelerated execution of the prescribed processing chains. The workload is representative of a real multi-process robotic system with several linear and nonlinear chains. 

%\emph{\blue R1.2 "Also, in Test 1, the number of priorities is equal to the number of streams offered by the GPU. Therefore, it looks like the thread-local priority queues are never solicited." } The new version of case study 1 shows a single- and multi- bucket 

\textbf{Review \#2:}
\emph{\blue R2.1. "Does a client represent an executor or a node or a callback with accelerator segment?" } Client is programmatically and syntactically a node, but the executor process is the sole entity issuing requests. The ROS2 nodal interface is simply a convenient data structure that overlays the executor.

\emph{\blue R2.2. "Does each registration request contain the information of all kernels used in a node (or an executor)? Does the registration response contain the shared memory IDs for all callbacks in a node (or an executor)?"" } During the registration request, the clients will list all anticipated kernels. The server process will generate and organize shared memory regions locally and respond with shared memory ID's. Once the client receives the shared memory id's for each kernel request type in the server's response, it will attach to them before modifying data and issuing requests.

\emph{\blue R2.3 "Is the shared memory allocated from each registration request used for multiple callbacks in (a node or an executor)?"} Callbacks of the same executor that require execution of multiples of the same kernel concurrently can issue multiple registration requests, one for each callback. Callback ID's are used during registration and are what is tracked/ managed by the server process.   

\textbf{Review \#3:}
\emph{\blue R3.1 "Another example is in Equation 1, where it is assumed that the communication cost (epsilon) is "callback independent”. The text does not justify how such cost is obtained and why it is independent of the data type or data size of a callback that request access to an accelerator."} We redefined $\epsilon$ to represent all overhead of AAMF, not just comm. cost. Sec.~\ref{sec:eval} includes the breakdown of $\epsilon$. Note that comm. cost is relatively constant due to zero-copy transfer of the data plane.

\emph{\blue R3.2 "The choices made for the case study (assignment of priorities and callbacks to CPUs) seem arbitrary and could therefore cause a positive bias on the outcome. Having such an arbitrary experiment on a single case study significantly reduces the external validity of the outcome of the experimental section of the paper."} The case study workloads are representative of a real robotic system and are not arbitrary. The parameters were chosen to showcase the benefit of using AAMF in both realistic and overloaded, but schedulable, scenarios. If we were to submit unschedulable critical chain configurations to the AAMF server, it would reject them as it would not be able to guarantee a response time. In case study 1, we purposefully assigned best effort chains to the same CPU-cores as the highest criticality chains. This was to show that, even under the most unfavorable conditions, AAMF would still guarantee response times. 

\emph{\blue R3.3 " Looking at the experimental results, (i) the response-time bounds derived for the chains when accessing to the hardware accelerators through the single interface is far larger than other solutions ... so it is not clear what is the gain in using the proposed framework, and (ii) the latency improvement gap (in comparison to not using a single interface) seems to be small."} We highlight that AAMF can bound the maximum response time of requests issued from various prioritized callback chains. The poorer, or marginally improved, performance of lower priority and best-effort accelerator-enabled callback chains is not a contribution of this paper. The framework specifically allows for coordinated accelerator access management that can allow for a a schedule system of critical callback chains to execute guaranteed latency bounds. 

\textbf{Review \#4:}
\emph{\blue R4.1. "the single accelerator limitation is a weak point. Multiple accelerator with multi-threading will make the work more substantial."} The AAMF framework supports multiple accelerators with multiple executing threads per accelerator. Recall that our GPU-specific implementation already uses multi-threading to execute requests preemptively.

%\emph{\blue R4.2. "The contribution is somewhat incremental. Real-time accelerator access management frameworks have been investigated before. This paper focuses on ROS 2."} Although real-time accelerator access management frameworks have been investigated, our work focuses on providing an 

